Collaborative causal inference with a distributed data-sharing management

Data sharing barriers are paramount challenges arising from multicenter clinical trials where multiple data sources are stored in a distributed fashion at different local study sites. Merging such data sources into a common data storage for a centralized statistical analysis requires a data use agreement, which is often time-consuming. Data merging may become more burdensome when causal inference is of primary interest because propensity score modeling involves combining many confounding variables, and systematic incorporation of this additional modeling in meta-analysis has not been thoroughly investigated in the literature. We propose a new causal inference framework that avoids the merging of subject-level raw data from multiple sites but needs only the sharing of summary statistics. The proposed collaborative inference enjoys maximal protection of data privacy and minimal sensitivity to unbalanced data distributions across data sources. We show theoretically and numerically that the new distributed causal inference approach has little loss of statistical power compared to the centralized method that requires merging the entire data. We present large-sample properties and algorithms for the proposed method. We illustrate its performance by simulation experiments and a real-world data example on a multicenter clinical trial of basal insulin treatment for reducing the risk of post-transplantation diabetes among kidney-transplant patients.

==> art/intro_diagram.tex <==

\begin{figure}
%  \hspace*{-2cm}\includegraphics[width=1.3\columnwidth,trim={0 10cm 0 6cm},clip]{Graphs_ENAR.eps}
    \figuresize{.25}
    \figurebox{10}{10}{}[art/Roundsdiagram.pdf]
    \caption{A diagram showing \oneR, \twoR, and \threeR\ procedures of the collaborative causal inference framework. Different types of arrows indicate the major updates involved in each round as shown in the legend. ATE which is short for Average Treatment Effect denotes the causal effect estimate.  
    %: solid arrows always involve propensity score (PS) updates;  dashed arrows indicate updating average treatment effect (ATE) estimates; dotted arrows represent incremental inference. 
    Panel a) shows \oneR\ evolves one round operation that updates PS, ATE and inferential quantities simultaneously. Panel b) shows \twoR\ involving two rounds of updates where the first round produces PS estimates, and the second round produces a causal effect and its variance. Panel c) shows \threeR\ involving three-rounds of updates.}
    \label{fig:my_label}
\end{figure}
% \begin{figure}
% \includegraphics[width=1.1\columnwidth]{figs/cpplot.eps}
%     \caption{A diagram showing Coverage probabilities of different algorithms in each scenario.}
%     \label{fig:my_label}
% \end{figure}


% \begin{figure}[H]
%     \centering


% \label{fig:fig1}


% \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

% % \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
% % %uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

% % %Shape: Rectangle [id:dp19467274572367943] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (77.5,95.93) -- (103.24,95.93) -- (103.24,123.42) -- (77.5,123.42) -- cycle ;
% % %U Turn Arrow [id:dp06067635520208192] 
% % \draw  [dash pattern={on 3.75pt off 3pt on 7.5pt off 1.5pt}] (88.26,95.8) -- (88.26,88.39) .. controls (88.26,86.57) and (89.74,85.09) .. (91.56,85.09) -- (135.11,85.09) .. controls (136.94,85.09) and (138.42,86.57) .. (138.42,88.39) -- (138.42,90.6) -- (139.49,90.6) -- (136.81,93.66) -- (134.13,90.6) -- (135.2,90.6) -- (135.2,88.39) .. controls (135.2,88.34) and (135.16,88.3) .. (135.11,88.3) -- (91.56,88.3) .. controls (91.51,88.3) and (91.47,88.34) .. (91.47,88.39) -- (91.47,95.8) -- cycle ;
% % %U Turn Arrow [id:dp4282143269440657] 
% % \draw  [dash pattern={on 3.75pt off 3pt on 7.5pt off 1.5pt}] (140.75,93.95) -- (140.75,87.21) .. controls (140.75,85.55) and (142.09,84.2) .. (143.75,84.2) -- (187.99,84.2) .. controls (189.65,84.2) and (191,85.55) .. (191,87.21) -- (191,89.22) -- (191.98,89.22) -- (189.54,92) -- (187.1,89.22) -- (188.08,89.22) -- (188.08,87.21) .. controls (188.08,87.16) and (188.04,87.13) .. (187.99,87.13) -- (143.75,87.13) .. controls (143.71,87.13) and (143.67,87.16) .. (143.67,87.21) -- (143.67,93.95) -- cycle ;
% % %U Turn Arrow [id:dp5002878625362621] 
% % \draw  [dash pattern={on 3.75pt off 3pt on 7.5pt off 1.5pt}] (195.13,94.29) -- (195.13,87.32) .. controls (195.13,85.6) and (196.53,84.2) .. (198.25,84.2) -- (234.85,84.2) .. controls (236.57,84.2) and (237.96,85.6) .. (237.96,87.32) -- (237.96,89.39) -- (238.97,89.39) -- (236.45,92.28) -- (233.92,89.39) -- (234.93,89.39) -- (234.93,87.32) .. controls (234.93,87.27) and (234.89,87.23) .. (234.85,87.23) -- (198.25,87.23) .. controls (198.2,87.23) and (198.16,87.27) .. (198.16,87.32) -- (198.16,94.29) -- cycle ;
% % %U Turn Arrow [id:dp6886265488106063] 
% % \draw  [dash pattern={on 3.75pt off 3pt on 7.5pt off 1.5pt}] (276.88,94.29) -- (276.88,87.32) .. controls (276.88,85.6) and (278.27,84.2) .. (279.99,84.2) -- (304.41,84.2) .. controls (306.13,84.2) and (307.53,85.6) .. (307.53,87.32) -- (307.53,89.39) -- (308.54,89.39) -- (306.01,92.28) -- (303.49,89.39) -- (304.5,89.39) -- (304.5,87.32) .. controls (304.5,87.27) and (304.46,87.23) .. (304.41,87.23) -- (279.99,87.23) .. controls (279.94,87.23) and (279.9,87.27) .. (279.9,87.32) -- (279.9,94.29) -- cycle ;
% % %U Turn Arrow [id:dp11254614871038382] 
% % \draw   (307.7,125.16) -- (307.7,133.81) .. controls (307.7,135.94) and (305.97,137.67) .. (303.84,137.67) -- (278.44,137.67) .. controls (276.31,137.67) and (274.58,135.94) .. (274.58,133.81) -- (274.58,131.24) -- (273.33,131.24) -- (276.46,127.66) -- (279.59,131.24) -- (278.34,131.24) -- (278.34,133.81) .. controls (278.34,133.87) and (278.38,133.92) .. (278.44,133.92) -- (303.84,133.92) .. controls (303.9,133.92) and (303.95,133.87) .. (303.95,133.81) -- (303.95,125.16) -- cycle ;
% % %U Turn Arrow [id:dp7474064894698926] 
% % \draw   (235.23,126.67) -- (235.23,134.69) .. controls (235.23,136.66) and (233.62,138.27) .. (231.65,138.27) -- (196.13,138.27) .. controls (194.15,138.27) and (192.55,136.66) .. (192.55,134.69) -- (192.55,132.3) -- (191.39,132.3) -- (194.29,128.99) -- (197.19,132.3) -- (196.03,132.3) -- (196.03,134.69) .. controls (196.03,134.74) and (196.07,134.79) .. (196.13,134.79) -- (231.65,134.79) .. controls (231.7,134.79) and (231.75,134.74) .. (231.75,134.69) -- (231.75,126.67) -- cycle ;
% % %U Turn Arrow [id:dp6214108251957413] 
% % \draw   (188.62,126.38) -- (188.62,134.6) .. controls (188.62,136.62) and (186.97,138.27) .. (184.95,138.27) -- (142.25,138.27) .. controls (140.22,138.27) and (138.58,136.62) .. (138.58,134.6) -- (138.58,132.15) -- (137.39,132.15) -- (140.36,128.75) -- (143.33,132.15) -- (142.14,132.15) -- (142.14,134.6) .. controls (142.14,134.65) and (142.19,134.7) .. (142.25,134.7) -- (184.95,134.7) .. controls (185,134.7) and (185.05,134.65) .. (185.05,134.6) -- (185.05,126.38) -- cycle ;
% % %U Turn Arrow [id:dp6676289314694182] 
% % \draw   (137.39,128.17) -- (137.39,135.15) .. controls (137.39,136.87) and (135.99,138.27) .. (134.27,138.27) -- (90.28,138.27) .. controls (88.56,138.27) and (87.17,136.87) .. (87.17,135.15) -- (87.17,133.08) -- (86.16,133.08) -- (88.68,130.19) -- (91.2,133.08) -- (90.2,133.08) -- (90.2,135.15) .. controls (90.2,135.2) and (90.23,135.24) .. (90.28,135.24) -- (134.27,135.24) .. controls (134.32,135.24) and (134.36,135.2) .. (134.36,135.15) -- (134.36,128.17) -- cycle ;
% % %Down Arrow [id:dp36282265139114855] 
% % \draw   (388.77,90.72) -- (390.3,89.39) -- (378.25,75.6) -- (381.3,72.94) -- (393.35,86.73) -- (394.88,85.39) -- (396.43,93.33) -- cycle ;
% % %Shape: Rectangle [id:dp7210534640785944] 
% % \draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][dash pattern={on 3.75pt off 3pt on 7.5pt off 1.5pt}] (144.97,58.5) -- (196,58.5) -- (196,78.33) -- (144.97,78.33) -- cycle ;
% % %Shape: Rectangle [id:dp6537684210080925] 
% % \draw  [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ] (144.79,142.7) -- (196.33,142.7) -- (196.33,163) -- (144.79,163) -- cycle ;
% % %Shape: Rectangle [id:dp5408401972790353] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (126.95,95.93) -- (152.69,95.93) -- (152.69,123.42) -- (126.95,123.42) -- cycle ;
% % %Shape: Rectangle [id:dp09617849027584047] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (175.98,95.93) -- (201.73,95.93) -- (201.73,123.42) -- (175.98,123.42) -- cycle ;
% % %Shape: Rectangle [id:dp5343581467883038] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (292.76,95.93) -- (318.5,95.93) -- (318.5,123.42) -- (292.76,123.42) -- cycle ;
% % %Shape: Rectangle [id:dp9463661331926414] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (405.72,92.47) -- (429.95,92.47) -- (429.95,118.03) -- (405.72,118.03) -- cycle ;
% % %Shape: Rectangle [id:dp5495817686500137] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (363.26,44.47) -- (387.49,44.47) -- (387.49,70.03) -- (363.26,70.03) -- cycle ;
% % %Shape: Rectangle [id:dp724038687226743] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (446.27,44.47) -- (470.5,44.47) -- (470.5,70.03) -- (446.27,70.03) -- cycle ;
% % %Down Arrow [id:dp7880401552551355] 
% % \draw   (438.38,85.56) -- (439.94,86.86) -- (451.63,72.77) -- (454.74,75.36) -- (443.05,89.45) -- (444.61,90.74) -- (437.02,93.54) -- cycle ;
% % %Shape: Rectangle [id:dp15916921420340646] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (365.26,140.47) -- (389.49,140.47) -- (389.49,166.03) -- (365.26,166.03) -- cycle ;
% % %Shape: Rectangle [id:dp24045677945615296] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (448.27,140.47) -- (472.5,140.47) -- (472.5,166.03) -- (448.27,166.03) -- cycle ;
% % %Down Arrow [id:dp7330223135447826] 
% % \draw   (447.26,121.73) -- (445.73,123.05) -- (457.71,136.9) -- (454.64,139.55) -- (442.66,125.7) -- (441.13,127.03) -- (439.62,119.08) -- cycle ;
% % %Down Arrow [id:dp6842535363592126] 
% % \draw   (397.63,126.64) -- (396.08,125.33) -- (384.32,139.36) -- (381.21,136.76) -- (392.98,122.73) -- (391.42,121.43) -- (399.03,118.67) -- cycle ;
% % %Shape: Rectangle [id:dp8747976589531903] 
% % \draw  [fill={rgb, 255:red, 222; green, 221; blue, 221 }  ,fill opacity=1 ] (224.98,95.93) -- (250.73,95.93) -- (250.73,123.42) -- (224.98,123.42) -- cycle ;
% % %U Turn Arrow [id:dp8641820196640331] 
% % \draw  [dash pattern={on 3.75pt off 3pt on 7.5pt off 1.5pt}] (238.45,93.28) -- (238.45,86.3) .. controls (238.45,85.34) and (239.22,84.56) .. (240.19,84.56) -- (273.64,84.56) .. controls (274.6,84.56) and (275.38,85.34) .. (275.38,86.3) -- (275.38,87.46) -- (275.97,87.46) -- (274.07,91.53) -- (272.18,87.46) -- (272.77,87.46) -- (272.77,87.17) .. controls (272.77,87.17) and (272.77,87.17) .. (272.77,87.17) -- (241.06,87.17) .. controls (241.06,87.17) and (241.06,87.17) .. (241.06,87.17) -- (241.06,93.28) -- cycle ;
% % %U Turn Arrow [id:dp2678890809121517] 
% % \draw   (272.58,125.16) -- (272.58,133.81) .. controls (272.58,135.94) and (270.86,137.67) .. (268.73,137.67) -- (243.33,137.67) .. controls (241.2,137.67) and (239.47,135.94) .. (239.47,133.81) -- (239.47,131.24) -- (238.22,131.24) -- (241.35,127.66) -- (244.47,131.24) -- (243.22,131.24) -- (243.22,133.81) .. controls (243.22,133.87) and (243.27,133.92) .. (243.33,133.92) -- (268.73,133.92) .. controls (268.78,133.92) and (268.83,133.87) .. (268.83,133.81) -- (268.83,125.16) -- cycle ;

% % % Text Node
% % \draw (84.08,101.16) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{1}};
% % % Text Node
% % \draw (268.29,100.46) node [anchor=north west][inner sep=0.75pt]   [align=left] {...};
% % % Text Node
% % \draw (131.56,172.84) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {incremental update};
% % % Text Node
% % \draw (373.03,175.45) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Meta-analysis};
% % % Text Node
% % \draw (149.4,63.25) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {Round 1};
% % % Text Node
% % \draw (149.79,145.7) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] { Round 2};
% % % Text Node
% % \draw (133.52,101.16) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{2}};
% % % Text Node
% % \draw (182.56,101.16) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{3}};
% % % Text Node
% % \draw (299.33,101.16) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{k}};
% % % Text Node
% % \draw (411.41,96.66) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{1}};
% % % Text Node
% % \draw (410.04,143.3) node [anchor=north west][inner sep=0.75pt]   [align=left] {...};
% % % Text Node
% % \draw (368.95,48.66) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{2}};
% % % Text Node
% % \draw (451.96,48.66) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{3}};
% % % Text Node
% % \draw (370.95,144.66) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{4}};
% % % Text Node
% % \draw (453.96,144.66) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{K}};
% % % Text Node
% % \draw (231.56,101.16) node [anchor=north west][inner sep=0.75pt]   [align=left] {S\textsubscript{4}};


% % \end{tikzpicture}
% % \caption{ A diagram contrasting the incremental update algorithm with the classic meta-analysis algorithm. K local sites are shown. The dashed arrow indicate the steps that sequentially update average treatment effect estimates and propensity score model estimates. The solid-line arrows indicate the distributive nature of meta-analysis approach }
%     \label{figure:my_label}



%     \centering

%     \caption{Caption}
%     \label{fig:my_label}

% \end{figure}




